On Nonconvex Optimization for Machine Learning: Gradients, Stochasticity, and Saddle Points

Gradient descent (GD) and stochastic gradient descent (SGD) are the workhorses of large-scale machine learning. While classical theory focused on analyzing the performance of these methods in convex optimization problems, the most notable successes in machine learning have involved nonconvex optimization, and a gap has arisen between theory and practice. Indeed, traditional analyses of GD and SGD show that both algorithms converge to stationary points efficiently. But these analyses do not take into account the possibility of converging to saddle points. More recent theory has shown that GD and SGD can avoid saddle points, but the dependence on dimension in these analyses is polynomial. For modern machine learning, where the dimension can be in the millions, such dependence would be catastrophic. We analyze perturbed versions of GD and SGD and show that they are truly efficient---their dimension dependence is only polylogarithmic. Indeed, these algorithms converge to second-order stationary points in essentially the same time as they take to converge to classical first-order stationary points.

==> proof_mb.tex <==
%!TEX root = main.tex


\section{Proof for Minibatch Case}

\cnote{Add simple arguement here.}


==> sketch.tex <==
%!TEX root = main.tex


\section{Proof of Deterministic Case}

\begin{algorithm}[ht]
\caption{Perturbed Gradient Descent (Easy to Analyze Version)}\label{algo:PGD_analysis}
\begin{algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input: }}
\renewcommand{\algorithmicensure}{\textbf{Output: }}
\REQUIRE $\x_0$, learning rate $\eta$, noise radius $r$.
\FOR{$t = 0, 1, \ldots, $}
\IF{$\norm{\grad f(\x_t)} \le  \epsilon$ and no perturbation in last $\utime$ iteration.}
\STATE $\x_t \leftarrow \x_t - \eta\xi_t \qquad \xi_t \text{~uniformly~} \sim B_0(r)$
\ENDIF
\STATE $\x_{t+1} \leftarrow \x_t - \eta \grad f (\x_t)$
\ENDFOR
\STATE \textbf{return} $\x_T$
\end{algorithmic}
\end{algorithm}

Let
\begin{equation} \label{eq:para_choice}
\eta = \frac{1}{\ell}, \qquad
\utime = \frac{\chi c}{\eta \sqrt{\rho\epsilon}},
\qquad
\ufun = \sqrt{\frac{\epsilon^3}{\rho}}\chi^{-3}c^{-5},
\qquad
r = \epsilon \chi^{-3}c^{-6}
\end{equation}
where $\chi = \max\{1, \log \frac{d \ell \Delta_f}{\rho\epsilon\delta}\}$


\begin{lemma}\label{lem:large_grad_GD}
Consider the setting of Theorem \ref{thm:main_GD}, if $\norm{\grad f(\x_t)} \ge \epsilon$, 
then by running GD, we have $f(\x_{t+1}) - f(\x_t) \le -\eta \epsilon^2/2$.
\end{lemma}
\begin{proof}
Immediately implied by Lemma \ref{lem:potential_decrease}.
\end{proof}

\begin{lemma}\label{lem:neg_curve_GD}
Consider the setting of Theorem \ref{thm:main_GD}, if $\norm{\grad f(\x_t)} \le \epsilon$
and $\lambda_{\min}(\hess f(\x_t)) \le -\sqrt{\rho\epsilon}$, 
then by adding perturbation then running GD, w.p. at least $1-\delta$, we have $f(\x_{t+\utime}) - f(\x_t) \le -\ufun$.
\end{lemma}
\begin{proof}
See next section.
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:main_GD}]
Combining lemma \ref{lem:large_grad_GD} and \ref{lem:neg_curve_GD}, we know
with probability $1-\frac{\Delta_f}{\ufun} \delta$, algorithm will find $\epsilon$-second order stationary point in following iterations:
\begin{align*}
\frac{\Delta_f}{\eta \epsilon^2} + \frac{\Delta_f \utime}{\ufun}
\le O(\frac{2\Delta_f }{\eta \epsilon^2}\chi^4)
\end{align*}
Let $\delta' = \frac{\Delta_f}{\ufun} \delta$ and substitute $\delta$ in $\chi$ with $\delta'$, we finished the proof.
\end{proof}

\subsection{Proof of Lemma \ref{lem:neg_curve_GD}}

\begin{lemma}\label{lem:potential_decrease}
Let $\eta \le \frac{1}{\ell}$, then we have GD satisfies:
\begin{equation*}
f(\x_{t+1}) - f(\x_{t}) \le -\frac{1}{2\eta}\norm{\x_{t+1} - \x_t}^2
\end{equation*}
\end{lemma}
\begin{proof}
By smoothness, we have:
\begin{align*}
f(\x_{t+1}) \le & f(\x_t) + \la\grad f(\x_t), \x_{t+1} - \x_t \ra + \frac{\ell}{2} \norm{\x_{t+1} - \x_t}^2 \\
 =& f(\x_t)  - \eta\norm{\grad f(\x_t)} + \frac{\eta^2\ell}{2} \norm{\grad f(\x_t)}^2
 \le f(\x_t) - \frac{\eta}{2}\norm{\grad f(\x_t)}^2 = f(\x_t) - \frac{1}{2\eta}\norm{\x_{t+1} - \x}^2
\end{align*}
\end{proof}

\begin{lemma}(Improve or Localize) \label{lem:locality}
Suppose $\{\x_t\}_{t=0}^T$ is a GD sequence, then
for all $t \le T$:
$$\norm{\x_t - \x_0} \le \sqrt{2\eta T(f(\x_0) - f(\x_T))}$$
\end{lemma}
\begin{proof}
By Cauchy-Swartz and Lemma \ref{lem:potential_decrease}, we have for all $t \le T$:
\begin{align*}
\norm{\x_t - \x_0} \le &\sum_{\tau = 1}^t \norm{\x_\tau - \x_{\tau - 1}}
\le \sqrt{T \sum_{\tau = 1}^t \norm{\x_\tau - \x_{\tau - 1}}^2}
\le \sqrt{ 2\eta T (f(\x_0) - f(\x_t))}
\end{align*}
Finally, since GD monotonically decrease function value, we have $f(\x_0) - f(\x_t) \le f(\x_0) - f(\x_T)$.
\end{proof}

Let $\text{GD}^{(t)}(\cdot)$ denote the update via GD $t$ times. Define Stuck region:
\begin{equation}
\cXs(\tilde{\x}) = \{\x | \x \in \ball_{\tilde{\x}}(\eta r), \text{~and~} f(\text{GD}^{(\utime)}(\x)) - f(\tilde{\x}) \ge -\ufun\}
\end{equation}

\begin{lemma}\label{lem:width}
There exists large enough constant $c$, so that if $\norm{\grad f(\tilde{\x})} \le \epsilon$
and $\lambda_{\min}(\hess f(\tilde{\x})) \le -\sqrt{\rho\epsilon}$, then the width of $\cXs(\tilde{\x})$ along 
the minimum eigenvector direction of $\tilde{\x}$ is at most $\delta \eta r \sqrt{2 \pi/d}$.
\end{lemma}

\begin{proof}
To prove this, let $\e_{\min}$ be the minimum eigenvector direction of $\hess f(\tilde{\x})$, it suffices to show for any $\x_0, \modify{\x}_0\in \ball_{\tilde{\x}}(\eta r)$ so that $\x_0 - \modify{\x}_0 = \lambda \e_{\min}$ where $|\lambda| \ge \delta \eta r \sqrt{2\pi/d}$, then either $\x_0 \not \in \cXs(\tilde{\x})$ or $\modify{\x}_0 \not \in\cXs(\tilde{\x})$.
To show $\x_0 \not \in \cXs(\tilde{\x})$ or $\modify{\x}_0 \not \in\cXs(\tilde{\x})$, by definition of stuck region it is equivalent to show:
\begin{equation*}
\min\{f(\x_\utime) - f(\tilde{\x}), f(\modify{\x}_\utime) - f(\tilde{\x})\} \le - \ufun
\end{equation*}
where $\x_\utime = \text{GD}^{(\utime)}(\x_0)$ and $\modify{\x}_\utime = \text{GD}^{(\utime)}(\modify{\x}_0)$.

In this proof, we will proceed by showing two steps:
\begin{enumerate}
\item $\max\{f(\x_0) - f(\tilde{\x}), f(\modify{\x}_0) - f(\tilde{\x})\} \le  \ufun$
\item $\min\{f(\x_\utime) - f(\x_0), f(\modify{\x}_\utime) - f(\modify{\x}_0)\} \le - 2\ufun$
\end{enumerate}
The final result immediately follow from triangle inequality.

\textbf{Part 1.} Since $\x_0 \in \ball_{\tilde{\x}}(\eta r)$ and $\norm{\grad f(\x)} \le \epsilon$, by smoothness, we have:
\begin{equation*}
f(\x_0) - f(\tilde{\x}) \le \epsilon \eta r + \frac{\ell}{2}(\eta r)^2
\le O(\frac{\epsilon^2}{\ell} \chi^{-3} c^{-6}) \le \ufun
\end{equation*}
The last inequality is due to $\ell/\sqrt{\rho\epsilon} \ge 1$, and constant $c$ large enough. By symmetry, we can also prove same upper bound for 
$f(\modify{\x}_0) - f(\tilde{\x})$.

~

\textbf{Part 2.} Assume the contradiction $\min\{f(\x_\utime) - f(\x_0), f(\modify{\x}_\utime) - f(\modify{\x}_0)\} \ge - 2\ufun$, by Lemma \ref{lem:locality}, this implies localization:
\begin{align*}
\forall t\le \utime, \quad &\max\{\norm{\x_t - \tilde{\x}}, \norm{\modify{\x}_t - \tilde{\x}}\} \\
\le& \max\{\norm{\x_t - \x_0} + \norm{\x_0 - \tilde{\x}}, \norm{\modify{\x}_t - \modify{\x}_0} + \norm{\modify{\x}_0 - \tilde{\x}}\} 
\le \sqrt{4\eta T\ufun}+ \eta r \le 4\sqrt{\frac{\epsilon}{\rho}} \chi^{-1} c^{-2}\defeq \uspace
\end{align*}
That is, both GD sequence $\{\x_t\}_{t=0}^{\utime}$ and $\{\modify{\x}_t\}_{t=0}^{\utime}$ will not leave a local ball with radius $\uspace$ around $\tilde{\x}$. Denote $\H = \hess f(\tilde{\x})$. By gradient update $\x_{t+1} = \x_t - \eta \grad f(\x_t)$, we can track the difference sequence $\w_t \defeq \x_t- \modify{\x}_t$ as:
\begin{align*}
\w_{t+1} =& \w_t -\eta [\grad f(\x_t) - \grad f(\modify{\x}_t)]
= (\I - \eta\H)\w_t - \eta \Delta_t \w_t \\
=& (\I - \eta\H)^{t+1}\w_0 - \eta\sum_{\tau = 0}^t(\I - \eta\H)^{t-\tau} \Delta_\tau \w_\tau 
\end{align*}
where $\H = \hess f(\tilde{\x})$ and $\Delta_t = \int_{0}^1 [\hess f(\modify{\x}_t + \theta (\x_t -\modify{\x}_t) - \H]\mathrm{d} \theta $. By Hessian Lipschitz, we have
$\norm{\Delta_t} \le \rho \max\{\norm{\x_t - \tilde{\x}}, \norm{\modify{\x}_t - \tilde{\x}} \} \le \rho\uspace$. We use induction to prove following:
\begin{align*}
\norm{\eta\sum_{\tau = 0}^{t-1}(\I - \eta\H)^{t-1-\tau} \Delta_\tau \w_\tau }
\le \frac{1}{2}\norm{(\I - \eta\H)^{t}\w_0}
\end{align*}
That is, the first term is always the dominating term.
Easy to check for base case $t=0$, we have $0 \le \norm{\w_0}/2$ the induction holds. Suppose for all $\modify{t} \le t$ the induction holds, this gives:
\begin{align*}
\norm{\w_{\modify{t}}} =
 \norm{(\I - \eta\H)^{\modify{t}}\w_0} + \norm{\eta\sum_{\tau = 0}^{\modify{t} - 1}(\I - \eta\H)^{\modify{t} - 1-\tau} \Delta_\tau \w_\tau} 
 \le 2\norm{(\I - \eta\H)^{\modify{t}}\w_0}
\end{align*}
Denote $\gamma = \lambda_{\min}(\hess f(\tilde{\x}))$, for case $t+1 \le \utime$, we have:
\begin{align*}
\norm{\eta\sum_{\tau = 0}^{t}(\I - \eta\H)^{t-\tau} \Delta_\tau \w_\tau }
\le& \eta\rho\uspace \sum_{\tau = 0}^{t} \norm{(\I - \eta\H)^{t-\tau}}\norm{\w_\tau} 
\le \eta\rho\uspace \sum_{\tau = 0}^{t} (1+\eta\gamma)^t \norm{\w_0}\\
\le &\eta\rho\uspace (t+1) \norm{(\I - \eta\H)^{t+1}\w_0}
\le \eta\rho\uspace\utime \norm{(\I - \eta\H)^{t+1}\w_0}
\le \frac{1}{2}\norm{(\I - \eta\H)^{t+1}\w_0}
\end{align*}
where the third last inequality use the fact $\w_0$ is along minimum eigenvector direction of $\H$,
the last inequality uses the fact $\eta\rho\uspace T =c^{-1} \le 1/2$ for $c$ large enough. Thus, we finishes the induction. 

Finally, we have:
\begin{align*}
\norm{\w_\utime} \ge& \norm{(\I - \eta\H)^{\utime}\w_0} - \norm{\eta\sum_{\tau = 0}^{\utime-1}(\I - \eta\H)^{\utime-1-\tau} \Delta_\tau \w_\tau }
\ge \frac{1}{2}\norm{(\I - \eta\H)^{\utime}\w_0}
\ge \frac{(1+\eta\sqrt{\rho\epsilon})^\utime \norm{\w_0}}{2}\\
=& 2^{\chi c} \cdot \frac{\delta \epsilon\chi^{-3}c^{-6}}{2\ell} \sqrt{\frac{2\pi}{d}} 
\ge 8\sqrt{\frac{\epsilon}{\rho}} \chi^{-1}c^{-2} = 2\uspace
\end{align*}
where the last inequality requires 
$$2^{\chi c} \ge \frac{16}{\sqrt{2\pi}} \cdot \frac{\ell \sqrt{d}}{\delta\sqrt{\rho \epsilon}} \chi^2 c^4$$
Since $\chi = \max\{1, \log \frac{d \ell \Delta_f}{\rho\epsilon\delta}\}$, it is easy to verify when $c$ large enough, above inequality holds. \cnote{More careful about the choice of $\chi$.}
% To make $\norm{\w_\utime} \ge 2\uspace$, 
% The choice of $\chi$ in Lemma \ref{lem:two_seq} gives $T  = \frac{\chi}{\eta\sqrt{\rho\epsilon}} \ge \frac{4}{\eta\sqrt{\rho\epsilon}} \log \frac{2}{\eta\rho r_0}$. 
% Since $2\eta\rho\uspace T \le 1$, we know
% $\frac{2}{\eta\rho r_0} \ge \frac{4\uspace T}{r_0}\ge\frac{4\uspace}{r_0}$. This implies
%  $T \ge \frac{4}{\eta\sqrt{\rho\epsilon}} \log \frac{4\uspace}{r_0}$, combined with $\eta\sqrt{\rho\epsilon} \le 1$, 
This gives $\norm{\w_\utime} \ge 2\uspace$
, which contradicts with the localization fact $\max\{\norm{\x_\utime - \tilde{\x}}, \norm{\modify{\x}_\utime - \tilde{\x}}\} \le \uspace$.

\end{proof}






\begin{proof}[Proof of Lemma \ref{lem:neg_curve_GD}]
Let $r_0 = \delta r \sqrt{\frac{2\pi}{d}}$ and applying Lemma \ref{lem:width}, we know $\cXs(\x_t)$ has at most width $\eta r_0$ in 
the minimum eigenvector direction of $\hess f(\x_t)$ and thus,
\begin{align*}
\text{Vol}(\cXs) \le \text{Vol}(\ball_0^{(d-1)}(\eta r)) \cdot \eta r_0
\end{align*}
which gives:
\begin{align*}
\frac{\text{Vol}(\cXs)}{\text{Vol}(\ball^{(d)}_{\x_t}(\eta r))}
\le \frac{\eta r_0 \times \text{Vol}(\ball^{(d-1)}_0(\eta r))}{\text{Vo{}l} (\ball^{(d)}_0( \eta  r))}
= \frac{r_0}{r\sqrt{\pi}}\frac{\Gamma(\frac{d}{2}+1)}{\Gamma(\frac{d}{2}+\frac{1}{2})}
\le \frac{r_0}{r\sqrt{\pi}} \cdot \sqrt{\frac{d}{2}+\frac{1}{2}} \le \delta
\end{align*}
This finishes the proof.
\end{proof}

% \begin{lemma}\label{lem:two_seq}
% Let $\tilde{\x}$ satisfies  $\lambda_{\min}(\hess f(\tilde{\x})) \le - \sqrt{\rho\epsilon}$.
% And $\x_0,  \modify{\x}_0$ are at most $r$ distance away from $\tilde{\x}$,
% $\w_0 =\x_0 -  \modify{\x}_0 = r_0 \e_1$ where $\e_1$ is the minimum eigenvector direction of $\hess f(\tilde{\x})$. 
% For any  $\chi \ge 4\log \frac{2}{\eta\rho r_0}$, let  $T  = \frac{\chi}{\eta\sqrt{\rho\epsilon}}$, $\ufun = \frac{1}{32\lt^3}\sqrt{\frac{\epsilon^3}{\rho}}$, and  $r$ satisfies $r \le \frac{1}{4\chi}\sqrt{\frac{\epsilon}{\rho}}$. Then we have:
% \begin{align*}
% \min\{f(\x_T) - f(\x_0), f(\modify{\x}_T) - f(\modify{\x}_0)\} \le - \ufun
% \end{align*}
% \end{lemma}
% \begin{proof}
% Assume the contrary, by Lemma \ref{lem:locality}, we know $\min\{E_T - E_0, \modify{E}_T - \modify{E}_0\} \ge - \ufun$ implies
% \begin{align*}
% \forall t\le T, \quad &\max\{\norm{\x_t - \tilde{\x}}, \norm{\modify{\x}_t - \tilde{\x}}\} \\
% \le& \max\{\norm{\x_t - \x_0} + \norm{\x_0 - \tilde{\x}}, \norm{\modify{\x}_t - \modify{\x}_0} + \norm{\modify{\x}_0 - \tilde{\x}}\} 
% \le \sqrt{2\eta T\ufun}+ r \defeq \uspace
% \end{align*}
% Denote $\H = \hess f(\tilde{\x})$. By gradient update $\x_{t+1} = \x_t - \eta \grad f(\x_t)$, we can track the difference $\w_t \defeq \x_t- \modify{\x}_t$ as:
% \begin{align*}
% \w_{t+1} =& \w_t -\eta [\grad f(\x_t) - \grad f(\modify{\x}_t)]
% = (\I - \eta\H)\w_t - \eta \Delta_t \w_t \\
% =& (\I - \eta\H)^{t+1}\w_0 - \eta\sum_{\tau = 0}^t(\I - \eta\H)^{t-\tau} \Delta_\tau \w_\tau 
% \end{align*}
% where $\H = \hess f(\tilde{\x})$ and $\Delta_t = \int_{0}^1 [\hess f(\modify{\x}_t + \theta (\x_t -\modify{\x}_t) - \H]\mathrm{d} \theta $. By Hessian Lipschitz, we have
% $\norm{\Delta_t} \le \rho \max\{\norm{\x_t - \tilde{\x}}, \norm{\modify{\x}_t - \tilde{\x}} \} \le \rho\uspace$. We use induction to prove following:
% \begin{align*}
% \norm{\eta\sum_{\tau = 0}^{t-1}(\I - \eta\H)^{t-1-\tau} \Delta_\tau \w_\tau }
% \le \frac{1}{2}\norm{(\I - \eta\H)^{t}\w_0}
% \end{align*}

% Easy to check for base case $t=0$, the induction holds. Suppose for all $\modify{t} \le t$ holds, this gives:
% \begin{align*}
% \norm{\w_{\modify{t}}} =
%  \norm{(\I - \eta\H)^{\modify{t}}\w_0} + \norm{\eta\sum_{\tau = 0}^{\modify{t} - 1}(\I - \eta\H)^{\modify{t} - 1-\tau} \Delta_\tau \w_\tau} 
%  \le 2\norm{(\I - \eta\H)^{\modify{t}}\w_0}
% \end{align*}
% Denote $\gamma = \lambda_{\min}(\hess f(\tilde{\x}))$, for case $t+1 \le T$, we have:
% \begin{align*}
% &\norm{\eta\sum_{\tau = 0}^{t}(\I - \eta\H)^{t-\tau} \Delta_\tau \w_\tau }
% \le \eta\rho\uspace \sum_{\tau = 0}^{t} \norm{(\I - \eta\H)^{t-\tau}}\norm{\w_\tau} \\
% \le &\eta\rho\uspace \sum_{\tau = 0}^{t} (1+\eta\gamma)^t \norm{\w_0}
% \le \eta\rho\uspace (t+1) \norm{(\I - \eta\H)^{t+1}\w_0}
% \end{align*}
% Therefore, as long as $2\eta\rho\uspace T \le 1$, we finishes the induction. By the condition for $\ufun$, $r$ in Lemma \ref{lem:two_seq}, it is easy to check that $2\eta\rho\uspace T = 2\eta\rho (\sqrt{2\eta T\ufun}+ r) T \le 1$ holds.
% Finally, we have:
% \begin{align*}
% \norm{\w_T} \ge \norm{(\I - \eta\H)^{T}\w_0} - \norm{\eta\sum_{\tau = 0}^{T-1}(\I - \eta\H)^{T-1-\tau} \Delta_\tau \w_\tau }
% \ge \frac{1}{2}\norm{(\I - \eta\H)^{T}\w_0}
% \ge \frac{(1+\eta\sqrt{\rho\epsilon})^T r_0}{2}
% \end{align*}
% The choice of $\chi$ in Lemma \ref{lem:two_seq} gives $T  = \frac{\chi}{\eta\sqrt{\rho\epsilon}} \ge \frac{4}{\eta\sqrt{\rho\epsilon}} \log \frac{2}{\eta\rho r_0}$. 
% Since $2\eta\rho\uspace T \le 1$, we know
% $\frac{2}{\eta\rho r_0} \ge \frac{4\uspace T}{r_0}\ge\frac{4\uspace}{r_0}$. This implies
%  $T \ge \frac{4}{\eta\sqrt{\rho\epsilon}} \log \frac{4\uspace}{r_0}$, combined with $\eta\sqrt{\rho\epsilon} \le 1$, this gives
% $\norm{\w_T} \ge \frac{2^{2 \log \frac{4\uspace}{r_0}} r_0}{2} \ge 2\uspace$
% , which contradicts with the fact $\max\{\norm{\x_T - \tilde{\x}}, \norm{\modify{\x}_T - \tilde{\x}}\} \le \uspace$.
% \end{proof}

% ~

% \begin{lemma}\label{lem:perturb_ball}
% Let $\tilde{\x}$ satisfies  $\norm{\grad f(\tilde{\x})}\le \epsilon$ and $\lambda_{\min}(\hess f(\tilde{\x})) \le - \sqrt{\rho\epsilon}$.
% Let $\{\x_t\}$ be the sequence of one-step perturbation of radius $r$ followed by gradient descent. 
% For any  $\chi \ge 4\log \frac{d}{\eta\rho \delta r}$, let  $T  = \frac{\chi}{\eta\sqrt{\rho\epsilon}}$, $\ufun = \frac{1}{32\lt^3}\sqrt{\frac{\epsilon^3}{\rho}}$, and $r$ satisfies $ r \le \frac{1}{200\chi^3 \sqrt{\cn}}\sqrt{\frac{\epsilon}{\rho}}$. Then, with probability at least $1-\delta$, we have:
% \begin{align*}
% f(\x_T) - f(\tilde{\x}) \le - \ufun/2
% \end{align*}
% \end{lemma}

% \begin{proof}
% The actual decrease in function can be decomposed into two parts:
% \begin{equation*}
% f(\x_T) - f(\tilde{\x}) = [f(\x_T) - f(\x_0)] + [f(\x_0)- f(\tilde{\x})]
% \le f(\x_T) - f(\x_0) + \epsilon r + \frac{\ell r^2}{2}
% \end{equation*}
% By the choice of $r$ in Lemma \ref{lem:perturb_ball}, it is easy to check $\epsilon r + \frac{\ell r^2}{2} \le \frac{\ufun}{2}$. 
% Define 
% $$\cXs = \{\x_0 | \x_0 \in \ball_{\tilde{\x}}(r) \text{~and~} f(\x_T) - f(\x_0) \ge -\frac{\ufun}{2}\}$$
% By
% \end{proof}

% \begin{proof}[Proof of Theorem \ref{thm:main}]
% Combining lemma \ref{lem:potential_decrease} and \ref{lem:perturb_ball}, we know
% with probability $1-\frac{\Delta_f}{\ufun} \tilde{\delta}$, algorithm will find $\epsilon$-second order stationary point in following iterations:
% \begin{align*}
% \frac{\Delta_f}{\eta \epsilon^2} + \frac{\Delta_f T}{\ufun}
% \le \frac{2\Delta_f }{\eta \epsilon^2}\chi^4
% \end{align*}
% Let $\delta = \frac{\Delta_f}{\ufun}\tilde{\delta}  = 32\Delta_f  \sqrt{\frac{\rho}{\epsilon^3}} \chi^3 \cdot \tilde{\delta}$.
% In Lemma \ref{lem:perturb_ball} we require $\chi \ge 4\log \frac{d}{\eta\rho \tilde{\delta} r}$, by pick 
% $r = \frac{1}{200\chi^3 \sqrt{\cn}}\sqrt{\frac{\epsilon}{\rho}} $ . The requirement becomes:
% \begin{align*}
% &\chi \ge 4 \log\left[\frac{d}{\eta\rho} \cdot \frac{32\Delta_f  \sqrt{\frac{\rho}{\epsilon^3}} \chi^3 }{\delta} 
% \cdot \frac{200\chi^3 \sqrt{\cn}}{\sqrt{\frac{\epsilon}{\rho}}}\right]\\
% \Leftarrow \quad &
% \chi - 12\log \chi \ge O\left(\log \frac{\Delta_f \cdot d\sqrt{\cn}}{\eta \epsilon^2\delta} \right)
% \end{align*}
% When $\chi \ge 200$, we have $\chi - 12 \log \chi \ge \frac{\chi}{2}$, by choice of learning rate $\eta = \frac{1}{\ell}$, this finishes the proof.


% \end{proof}

